Continual Deep Learning by Functional Regularisation of Memorable Past

Continually learning new skills is important for intelligent systems, yet standard deep learning methods suffer from catastrophic forgetting of the past. Recent works address this with weight regularisation. Functional regularisation, although computationally expensive, is expected to perform better, but rarely does so in practice. In this paper, we fix this issue by using a new functional-regularisation approach that utilises a few memorable past examples crucial to avoid forgetting. By using a Gaussian Process formulation of deep networks, our approach enables training in weight-space while identifying both the memorable past and a functional prior. Our method achieves state-of-the-art performance on standard benchmarks and opens a new direction for life-long learning where regularisation and memory-based methods are naturally combined.

==> sections/4toy_experiments.tex <==
In Appendix~\ref{app:toydata}, we use a 2D binary classification toy dataset with a small MLP to (i) demonstrate the brittleness and inconsistent behaviour of weight-regularisation, (ii) test FROMP's performance when exposed to different toy datasets of varying difficulty. 
As shown in Appendix~\ref{app:toydata}, we find that weight-regularisation methods such as VCL perform much worse than functional-regularisation, with lower accuracy, higher variance over random seeds, and visually bad decision boundaries.
